Weld: Rethinking the Interface Between Data-Intensive Applications

Data analytics applications combine multiple functions from different libraries and frameworks. Even when each function is optimized in isolation, the performance of the combined application can be an order of magnitude below hardware limits due to extensive data movement across these functions. To address this problem, we propose Weld, a new interface between data-intensive libraries that can optimize across disjoint libraries and functions. Weld exposes a lazily-evaluated API where diverse functions can submit their computations in a simple but general intermediate representation that captures their data-parallel structure. It then optimizes data movement across these functions and emits efficient code for diverse hardware. Weld can be integrated into existing frameworks such as Spark, TensorFlow, Pandas and NumPy without changing their user-facing APIs. We demonstrate that Weld can speed up applications using these frameworks by up to 29x.

==> backends.tex <==
%!TEX root=nvl.tex
\section{Hardware Backends}
\label{sec:backends}

In this section, we sketch the main challenges tackled in each backend.

\subsection{Multi-Threaded CPU Backend}
\label{sub:backend-cpu}

The execution engine is based on techniques from~\cite{tzannes2010lazy},
and avoids the per-workload parameter tuning required in more general
parallel runtimes like Cilk~\cite{cilk}.

The execution engine represents a \sn program as a linear task graph with each
outer \lstinline$for$ loop represented as a single task that is a dependency
of all loops and statements that come after it. A loop can only execute after
its dependencies. The engine creates a worker thread for each core and a task queue
for each worker, where a task consists of a range of loop iterations.
Initially, all iterations of the first loop are given to the first worker. Loops are
split into multiple tasks to load-balance work; a worker steals tasks from other workers'
queues when idle. An executing worker creates a new task with half its remaining
iterations for the current loop when it observes that its own task queue is
empty. Tasks for nested loops are created by splitting the outermost loop with
more than one iteration remaining; this policy ensures that expensive inner
loops will be split across cores, but smaller inner loops will not
incur task creation overhead.

Much of our flexibility in the parallel
builder design, in particular our ability to maintain per-thread data structures
until a \lstinline$result$ call, is due to the \textit{write-only, build-once}
specification of the builder contract.

\subsection{GPGPU Backend}
\label{sub:backend-gpu}

GPUs excel at problems with significant data parallelism such as
relational queries or computation over collections of vectors. Our GPU
backend is a restricted prototype for the subset of the \sn \il that
is likely to yield performance benefits compared to CPUs (avoiding
tricky cases such as the construction of dictionaries using
dictmergers). This backend translates \sn{} programs into
Voodoo~\cite{voodoo}, a virtualization layer over OpenCL. Even in the
limited subset of the language we ported, there are two performance
challenges with respect to efficient computing results: flattening
nested data structures and massively parallel (hierarchical) merging
of values into builders.

\noindent{\bf Unnesting.}
Since GPUs do not support dynamic memory allocation or pointers,
nested vectors must be flattened. We apply a similar unnesting process
to the one described in~\cite{blelloch1988compiling}: we concatenate
the nested vectors and keep a secondary vector containing the offsets
of the beginnings of each of the nested vectors (similar to
  the compressed sparse row representation of a matrix). At runtime,
iterations over the nested vectors are translated into iterations over
the subranges of the flattened vector -- each subrange is mapped to an
OpenCL thread. SIMT GPUs experience performance penalties when vector sizes
are skewed. We thus partition vectors into batches of no more than 128 elements and
maintain a third vector that maps the original vector to its partition.

\noindent{\bf Massively Parallel Merging.}
Since builders form the core of \sn, their efficient implementation is
imperative. As with the multicore backend, there are two design options: a
shared data structure protected by atomic instructions or a partitioned per-core
data structure that is merged when a result is produced. We select the strategy
based on the (estimated) cardinality of the output: shared data structures for high
cardinalities, hierarchical  merges for low cardinalities. While the
partition granularity of the merge is a (statically) tunable parameter, we found
that processing 4096 scalar values per work item (and parallelizing the work
items) consistently yields good performance.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nvl"
%%% End:


==> language-details.tex <==
%!TEX root=nvl.tex

\section{\sn \il Details}
\label{sec:language-details}
Table~\ref{table:operators} shows a detailed specification of the operators
available in \sn.  The core language consists of a small number of basic
operators (top table).  On top of these, we have also provided ``sugar''
operators for functional programming implemented as macros that map into
\lstinline$for$ loops and builders.

\sn can also represent SIMD vectors using struct data types composed of the
same type.  For example, \lstinline${int,int,int,int}$ represents a four-wide
128-bit vector register.

\;\;

\begin{table*}[t]
\centering
\small
\begin{tabular}{|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{Core Operators in \sn}}                                                                                                           \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{Basic Operators}}} & Arithmetic expressions: \lstinline$a + b, -a, a & b$, etc.                                 \\ \cline{2-2}
\multicolumn{1}{|c|}{}                                           & Let expression: \lstinline$name := expr; body$, to assign variable names                    \\ \cline{2-2}
\multicolumn{1}{|c|}{}                                           & \lstinline$if(condition) on_true else on_false$                                                  \\ \cline{2-2}
                                                                 & \lstinline$while(init, update)$: sequentially loops \lstinline$update$ function starting from an initial value     \\ \cline{2-2}
                                                                 & \lstinline$bitselect(cond, true, false)$: evaluates \lstinline$true$ and \lstinline$false$ and chooses based on the bit \lstinline$cond$.      \\ \cline{2-2}
                                                                 

             & \lstinline$call(func, args)$ calls an existing serial C function. \\ \hline
                                                                 
                                                                 
\multirow{5}{*}{\textbf{Collection Operators}}
                                                                 & \lstinline$lookup(vector, index)$ and \lstinline$lookup(dictionary, key)$           \\ \cline{2-2}
                                                                 & \lstinline$struct.0, struct.1$, etc.~to access fields in a struct                   \\ \cline{2-2}
                                                                 & \lstinline$len(vector)$ and \lstinline$len(dictionary)$                             \\ \cline{2-2}
                                                                 & \lstinline$sort(vector, keyfunc)$ to sort a vector based on the key returned by \lstinline$keyfunc$   \\ \cline{2-2}
                                                                 & \lstinline$tovec(dictionary)$ to get entries of a dictionary as a \lstinline$vec[K,V]$              \\ \hline

\multirow{3}{*}{\textbf{Builder Operators}}
                    & \lstinline$merge(builder, elem)$ to merge one value into a builder  \\ \cline{2-2}
                    & \lstinline$result(builder)$ to get a result from a builder   \\ \cline{2-2}
                     & \lstinline$for(vector, builders, func)$ to loop over a vector in parallel (\S\ref{sub:operators}) \\ \hline
\end{tabular}

\;\;

\begin{tabular}{|p{0.726\textwidth}|}
  \hline
  \multicolumn{1}{|c|}{\textbf{Functional Sugar Operators}} \\ \hline
  \lstinline$map(v: vec[T], f: T => U): vec[U]$ \\ \hline
  \lstinline$flatmap(v: vec[T], f: T => U): vec[U]$ \\ \hline
  \lstinline$filter(v: vec[T], f: T => bool): vec[T]$ \\ \hline
  \lstinline$reduce(v: vec[T], id: T, f: (T, T) => T): T$ \\ \hline
  \lstinline$zip(v1: vec[T1], v2:...)$ \lstinline$: vec[{T1, T2, ...}]$ \\ \hline
  \lstinline$groupby(v: vec[T], key: T => K, val: T => V)$ \lstinline$: dict[K, vec[V]]$ \\ \hline
\end{tabular}

\;\;

\centering
\caption{Operators available in \sn. The top table shows the core built-in operators, while the bottom table shows ``sugar'' operators for functional programming implemented as macros using \lstinline$for$ loops and builders.}
\label{table:operators}
\end{table*}



==> udfs.tex <==
\section{UDFs in \sn}
\label{sec:udfs}

\rthree{

\sn's \il supports arbitrary C UDFs which can take any data type as input.
Library writers specify the parameter types and return type of the UDF, and the
C function is responsible for understanding the in-memory structure \sn uses
(\eg structs are packed C structs, vectors are 2-tuples of data
pointer and  length, \etc). \sn interprets the return value of the UDF using
the specified return type.

\paragraph{Python UDFs.}



We analyze Python ASTs using methodologies similar to prior
work such as Tupleware~\cite{tupleware} and Pydron~\cite{pydron}. We use the Meta~\cite{meta} library to decompile a
Python expression into an AST. Each node in the  AST is mapped to a
corresponding \sn expression. The translator can parse arithmetic expressions,
lists, structs (represented as Python tuples), Python's builtin functional
expressions (\eg \lstinline$map$ and \lstinline$reduce$), and indexing into
lists and structs using Python's subscripting syntax. Nested data types can
also be captured (\eg lists of lists). If the translator finds an AST node it
cannot parse (\eg a print statement), it returns an error. Dictionaries are not
supported.

To help the system, users must annotate functions with a type
signature, designating the type of each input argument as well as the return
value. Because \sn is a functional language where each expression is a pure
function of its subexpressions, the types of other intermediate variables
within the function can be inferred using just the return type and the argument types.
Our translator does not currently support generic functions; each function must have
a concrete type signature.
}

